Incremental 3D Semantic Scene Graph Prediction from RGB Sequences

3D semantic scene graphs are a powerful holistic representation as they describe the individual objects and depict the relation between them. They are compact high-level graphs that enable many tasks requiring scene reasoning. In real-world settings, existing 3D estimation methods produce robust predictions that mostly rely on dense inputs. In this work, we propose a real-time framework that incrementally builds a consistent 3D semantic scene graph of a scene given an RGB image sequence. Our method consists of a novel incremental entity estimation pipeline and a scene graph prediction network. The proposed pipeline simultaneously reconstructs a sparse point map and fuses entity estimation from the input images. The proposed network estimates 3D semantic scene graphs with iterative message passing using multi-view and geometric features extracted from the scene entities. Extensive experiments on the 3RScan dataset show the effectiveness of the proposed method in this challenging task, outperforming state-of-the-art approaches.

==> tables/segment_recall.tex <==
\begin{table}
    \centering
    \begin{tabular}{c|ccc}
         & \emph{GT} & \emph{Dense} & \emph{Sparse} \\
         \hline
         Recall(\%) & 100 & 76.9 & 47.2\\
    \end{tabular}
    \caption{The entity recall on different input methods. \emph{Dense} is with the incremental segmentation from \cite{Tateno2015}. \emph{Sparse} is our IEE pipeline.}
    \label{tbl:segment_recall}
\end{table}

==> tables/ssg_3RScan_ScanNet20_PerPredicate.tex <==
    \begin{table*}
    \centering
    % \resizebox{\textwidth}{!}{
    \begin{tabular}{c|c|c|c|c|c|c|c|c|c|c|}
         & & attached to & build in & connected to & hanging on & none & part of & standing on & supported by & avg \\
\hline
\multirow{5}{*}{\rotatebox{90}{\emph{GT}}} 
&IMP&
0.552 & 0.154 & 0.271 & 0.116 & 0.983 & 0.250 & 0.724 & 0.000 & 0.381\\%IMP_full_l20_6
&VGfM&
0.650 & 0.231 & 0.375 & 0.232 & 0.980 & 0.312 & 0.784 & 0.000 & 0.446\\%VGfM_full_l20_8
&3DSSG&
0.711 & 0.667 & 0.292 & 0.486 & 0.976 & 0.688 & 0.833 & 0.044 & 0.587\\%3DSSG_full_l20_3
&SGFN&
0.736 & 0.769 & 0.521 & 0.594 & 0.965 & 0.812 & 0.823 & 0.022 & 0.655\\%SGFN_full_l20_2
% &2DSSG&
% 0.779 & 0.974 & 0.792 & 0.913 & 0.935 & 0.562 & 0.876 & 0.187 & 0.752\\%2DSSG_full_l20_4
&Ours&
0.766 & 0.795 & 0.708 & 0.681 & 0.969 & 0.812 & 0.914 & 0.077 & 0.715\\%JointSSG_full_l20_4
\hline
\multirow{5}{*}{\rotatebox{90}{\emph{Dense}}} 
&IMP&
0.473 & 0.026 & 0.229 & 0.051 & 0.969 & 0.000 & 0.014 & 0.077 & 0.230\\%IMP_INSEG_l20_3
&VGfM&
0.531 & 0.051 & 0.146 & 0.123 & 0.971 & 0.000 & 0.005 & 0.121 & 0.244\\%VGfM_inseg_l20_1
&3DSSG&
0.594 & 0.205 & 0.083 & 0.152 & 0.944 & 0.000 & 0.010 & 0.143 & 0.266\\%3DSSG_INSEG_l20_3
&SGFN&
0.603 & 0.205 & 0.250 & 0.203 & 0.959 & 0.062 & 0.006 & 0.154 & 0.305\\%SGFN_inseg_l20_0
% &2DSSG&
% 0.611 & 0.333 & 0.417 & 0.297 & 0.941 & 0.000 & 0.002 & 0.110 & 0.339\\%2DSSG_inseg_l20_0
&Ours&
0.628 & 0.308 & 0.312 & 0.283 & 0.958 & 0.000 & 0.012 & 0.132 & 0.329\\%Joint_inseg_l20_0
\hline
\multirow{5}{*}{\rotatebox{90}{\emph{Sparse}}}
 & IMP & 0.169 & 0.000 & 0.021 & 0.022 & 0.990 & 0.000 & 0.014 & 0.011 & 0.153\\%IMP_orbslam_l20_i
 & VGfM & 0.183 & 0.000 & 0.000 & 0.007 & 0.990 & 0.000 & 0.004 & 0.022 & 0.151\\%VGfM_orbslam_l20_1
 & 3DSSG & 0.178 & 0.000 & 0.021 & 0.029 & 0.964 & 0.062 & 0.014 & 0.011 & 0.160\\%3DSSG_3rscan_orbslam_l20_0
 & SGFN & 0.134 & 0.000 & 0.000 & 0.000 & 0.984 & 0.000 & 0.012 & 0.011 & 0.143\\%SGFN_3rscan_orbslam_l20_0
 % & 2DSSG & 0.205 & 0.077 & 0.104 & 0.123 & 0.976 & 0.062 & 0.016 & 0.011 & 0.197\\%2DSSG_orbslam_l20_0
 & JointSSG & 0.200 & 0.026 & 0.000 & 0.065 & 0.984 & 0.000 & 0.017 & 0.011 & 0.163\\
 
 
    \end{tabular}
    % }
    \caption{Caption}
    \label{tbl:ssg_3RScan_ScanNet20_PerPredicate}
\end{table*}
